ViT5: Pretrained Text-to-Text Transformer for Vietnamese Language Generation

We present ViT5, a pretrained Transformer-based encoder-decoder model for the Vietnamese language. With T5-style self-supervised pretraining, ViT5 is trained on a large corpus of high-quality and diverse Vietnamese texts. We benchmark ViT5 on two downstream text generation tasks, Abstractive Text Summarization and Named Entity Recognition. Although Abstractive Text Summarization has been widely studied for the English language thanks to its rich and large source of data, there has been minimal research into the same task in Vietnamese, a much lower resource language. In this work, we perform exhaustive experiments on both Vietnamese Abstractive Summarization and Named Entity Recognition, validating the performance of ViT5 against many other pretrained Transformer-based encoder-decoder models. Our experiments show that ViT5 significantly outperforms existing models and achieves state-of-the-art results on Vietnamese Text Summarization. On the task of Named Entity Recognition, ViT5 is competitive against previous best results from pretrained encoder-based Transformer models. Further analysis shows the importance of context length during the self-supervised pretraining on downstream performance across different settings.

==> sections/methods.tex <==
Following the works descried in \cite{attention}, a transformer-based sequence-to-sequence architecture is an encoder-decoder architecture that has multi-layer self-attention. This architecture consists of two components: an encoder and a decoder.
    % \begin{itemize}
    %     \item The encoder captures contextualized representation of the input sequence
    %     \item The decoder will use this contextualized representation to generate the target sequence
    % \end{itemize}

Therefore, in order to generate a target sequence from an input sequence, a full transformer architecture with both an encoder and a decoder is required. PhoBERT and ViBERT are encoder-only models developed for encoding Vietnamese Language representations, so we can quickly assemble these models into the architecture. However, for the decoder level, we change the self-attention layers from bidirectional into left-context-only. We also insert a randomly initialized cross-attention mechanism into the decoder. We denote these models as PhoBERT2PhoBERT and ViBERT2ViBERT. Following the practice from \cite{press-wolf-2017-using}, we tie the input embedding and output embedding in the decoder block, allowing the model to learn from the input embedding weights instead of random weights.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\textwidth,keepaspectratio]{section/PhoBERT2PhoBERT.pdf}
%     \caption{Transformer-based encoder-decoder architecture}
%     \label{fig:model}
% \end{figure*}

For existing encoder-decoder models like mT5, mBART, and BARTpho, we continuously fine-tune on the released checkpoints while strictly keeping their structure and vocabulary.

We test the models on two single document abstractive summary datasets (Wikilingua \cite{wikilingual} and Vietnews \cite{vietnews}) and one multi-document summarization dataset (ViMS \cite{vims}). The statistics for these datasets are shown in Table \ref{data}.

% We give an overview of the Transformer-based encoder-decoder architecture in Fig \ref{fig:model}. In this overview, we show the process for condensing a long Vietnamese text sequence (\textit{Ex: He took a taxi to attend a party in a fancy restaurant. While in the party, he collapsed and was rushed to the hospital}) to a short summary (\textit{Ex: He was hospitalized after attending a party}).



==> sections/metrics.tex <==
\subsubsection{Summarization Metrics}
We use ROUGE Score as our benchmark metrics for both single document summarization dataset. ROUGE (Recall-Oriented Understudy for Gisting Evaluation) measures the number of overlapping units (including n-grams and word sequences) between two sequences. We use ROUGE-1, ROUGE-2, and ROUGE-L, which are the overlap between unigrams, bigrams, and longest matching sequence.

We use \textbf{ROUGE} \cite{rouge} which has been applied to text generation, summarization, standard machine translation metrics, and other miscellaneous performance statistics to be our evaluation method. 
\begin{itemize}

    \item BERTScore \cite{bertscore} is an evaluation metric for text generation. BERTScore measures token similarity score for each token between two sequences using contextual embeddings. We choose BERTScore for its recent adaption as a language model-based text generation metric. For the purpose of fair benchmarking, we will compute BERTScore by using Multilingual BERT \cite{bert}

\end{itemize}





\begin{itemize}
    \item \textbf{ROUGE-N: } measures overlap between unigrams, bigrams, trigrams and higher order n-grams For our experiments, we will use ROUGE-1 and ROUGE-2 (unigrams and bigrams)
    \item \textbf{ROUGE-L: } measures longest matching sequence of words using Longest Common Subsequences (LCS) with the assumption that longer LCS between the generated summary and the reference summary shows more similarity (higher quality of results).
     This variant of ROUGE compares the system
generated summary and the human generated summary
based on the Longest Common Subsequences (LCS)
between them. The premise is that, longer LCS between
the system and human summaries shows more similarity
and therefore higher quality of the system summary
\end{itemize}

==> sections/models.tex <==
\subsection{BERT}
BERT \cite{bert} (Bidirectional Encoder Representations from Transformers) is a multilayer bidirectional Transformer encoder based on the architecture described in \cite{attention}. In BERT, each input sequence is represented by a sum of the  token embeddings, segment embeddings, its positional embeddings. BERT uses the WordPiece tokenizer to split words into subwords. 


\subsection{PhoBERT}
PhoBERT \cite{phobert} is the first public large-scale mongolingual language model pretrained for Vietnamese. PhoBERT follows the architecture proposed by \cite{roberta}. The PhoBERT pretraining approach is also based on RoBERTa \cite{roberta}, employing the implementation in \textit{fairseq} \cite{fairseq} which optimizes the BERT pretraining procedure for more robust performance. The model is trained on a 20GB word-level Vietnamese news corpus with maximum sequence length of 256.

\subsection{ViBERT}
ViBERT \cite{vibert} leverages checkpoints from the multilingual pretrained model mBERT \cite{bert} and continues training on monolingual Vietnamese corpus (10GB of syllable-level text). The authors also remove insignificant vocab from mBERT, keeping only Vietnamese vocab. 


\subsection{mBERT}
mBERT followings the same training procedure of BERT \cite{bert} on a multilingual dataset. The training languages are the 100 languages with the largest amount of text on Wikipedia, which includes Vietnamese \footnote{https://meta.wikimedia.org/wiki/List\_of\_Wikipedias}.


\subsection{mBART}
mBART \cite{mbart} is a sequence-to-sequence denoising encoder-decoder model that was pretrained on large-scale monolingual corpora (including Vietnamese) using the BART objective anđ architecture \cite{bart}.
% BART follows sequence-to-sequence Transformer architecture from \cite{attention}, except a GeLUs \cite{gelu} activation functions is used instead of ReLU. 
% BART architecture is closely related to that of BERT, with the following differences:
%     \begin{itemize}
%         \item Each layer of the decoder performs cross-attention over the final hidden layer of the encoder (following \citet{attention})
%         \item BART does not have an additional feed-forward network before word prediction
%     \end{itemize}

\subsection{mT5}
mT5 \cite{mT5} is a multilingual variant of the large pretrained encoder-decoder text-to-text models T5 \cite{t5}. 
% T5 explores the landscape of transfer learning techniques for NLP by training a model on an massive corpus (800GB of text) and introducing a unified framework that converts all text-based problems into a text-to-text format. 
mT5 inherits all of the benefits of T5 including the scale and the design which was based on a large-scale empirical study \cite{t5}.

\subsection{BARTpho}
BARTpho is the first and most recently released large-scale monolingual sequence-to-sequence models pretrained for Vietnamese. It follows the architecture and pretraining scheme of the sequence-to-sequence denoising model BART. The authors release two version of BARTpho: syllable-level and word-level input texts, called BARTpho$_{syllable}$ and BARTpho$_{word}$ respectively.




==> sections/multidoc.tex <==
\input{ACLStudent2021/table/vimds_stats}


In this section, we will propose a Bi-Encoder-Decoder architecture for sequence-to-sequence models in generating summarization in multi-document setting. Our proposed architecture works for both extractive summarization and abstractive summarization tasks. We benchmark multi-Document extractive summarization on the VietnameseMDS\footnote{https://github.com/lupanh/VietnameseMDS} dataset with current works and methods from \citet{to2021monolingual}. Because studies in large monolingual Vietnamese Encoder-Decoder models are limited, we propose and apply our architecture as the baseline for abstractive summarization on the same VietnameseMDS dataset.
\subsection{VietnameseMDS Multi-Document Summarization Dataset}
The dataset contains 200 clusters, each containing documents related to a topic. These documents are news articles\footnote{https://baomoi.com}. Each cluster has 3-5 documents and 2 human labelled reference summarization of these articles. Statistics of the dataset is shown in Table \ref{vimds_stats}. Each reference has an average of 182 words.

\subsection{Bi-Encoder-Decoder Architecture}
We propose a Bi-Encoder-Decoder architecture to generate extractive summary and abstractive summary text. A list of sentences will be fed into a pre-trained encoder to produce meaningful embeddings of these sentences. In the other encoder, an embedding of summary/reference is returned by the model. We will then compute the similarity between each of these sentence embeddings and the reference summaries embedding(s). Using cosine-similarity (or can be substituted with Manhattan/Euclidean distance), semantically meaningful sentences to a reference summary can be retrieved. The K most meaningful sentences will be concatenated into one simple document. This cluster of K most similar sentence(s) is used as extractive summarization context.

This generated single document will be treated as one long embedding and fed into the decoder layers to generate texts. These outputs are the abstractive summary of a respective input sample. The architecture layout is in Figure \ref{fig:biencoderdecoder}.

\begin{figure*}[hbt!]
    \centering
    \includegraphics[width=0.9\textwidth,height=0.5\textheight,keepaspectratio]{ACLStudent2021/figures/biencoderdecoder.drawio.pdf}
    \caption{The Bi-Encoder-Decoder architecture}
    \label{fig:biencoderdecoder}
\end{figure*}


\subsection{Experiments and Results}
\subsubsection{Extractive Summarization}
\label{extractive_summarization}
The authors of \citet{to2021monolingual} used K-means clustering to filter out embedded sentences from the BERT embedding layer. K-means algorithm chooses the most embedded sentences that are closest to the centroids of the documents. The work did experiments on the VietnameseVMDS dataset with both multilingual and monolingual Vietnamese BERTs. The works only report Rouge-1 and Rouge-2 scores on the benchmark. Therefore, we will only report Rouge scores in this task.

Following our Bi-Encoder-Decoder architecture in Figure \ref{fig:biencoderdecoder}, we do sentence tokenizing of all the sentences in the documents and use cosine-similarity to extract the top K meaningful sentences compared to the summary embeddings. These embeddings are concatenated to construct one single document and benchmark with the gold reference. The results are shown in Table \ref{extractive_result}

Using normal BERT encoders with K-means clustering to generate embeddings achieves stable performance on the extractive summarization task, as the results from mBERT, PhoBERT, and viBERT4news\footnote{https://huggingface.co/NlpHUST/vibert4news-base-cased} are roughly competitive.  There is minor improvement in PhoBERT\textsubscript{large} from PhoBERT\textsubscript{base} in Rouge-1 (~0.4\%) while Rouge-2 scores are approximately the same. Because multilingual mBERT still performs better than base monolingual PhoBERT, we believe that there are still opportunities using monolingual encoder to excel in extractive summarization tasks.

Utilizing Bi-Encoder with cosine-similarity function, there is a significant difference in performance between BART-based architecture models and T5-based architecture models; mT5 multilingual model performs better than mBART across all metrics; leading to an assumption that T5-architecture's encoder is more effectively in Bi-Encoder setting. This assumption is more clearly shown in the performance of monolingual BARTpho and our ViT5 models. The Bi-Encoder of BARTpho performs worst on the tasks with ~3\% lower than its multilingual version across all Rouge metrics.

The ViT5 models-encoder achieve state-of-the-art results on extractive summarization. Both version of ViT5\textsubscript{256-length} and ViT5\textsubscript{1024-length} excel and achieve highest result in Rouge-1, Rouge-2, and Rouge-L. The significant increasing in ViT5's performance compared to mT5 shows that pre-training Encoder-Decoder models in Vietnamese monolingual setting gives the sequence-to-sequence model a better understanding and learning context representation between two embeddings sentences more effectively. The quality and length of training data during self-supervised training also give ViT5\textsubscript{1024-length} model a better performance in extracting context representation between documents and summary reference.

\input{ACLStudent2021/table/extractive_result}
\subsubsection{Abstractive Summarization}
The results of VietnameseMDS multi-document abstractive summarization are shown in Table \ref{abstractive_result}. 
We divide train/dev/test split as 0.7/0.1/0.2 respectively; this will be released concurrently with our code implementation for the purpose of reproducing the work. 

Pre-trained multilingual models (mBART and mT5) achieve competitive results on the abstractive generation; mBART achieves second best score on Rouge 1 and mT5 achieves second best scores on Rouge 2 and Rouge L. BARTpho, a monolingual pre-trained on the same setting as mBART \cite{bartpho, mbart}, surprisingly performs worse than its multilingual version. This can be attributed to the bad performance of BARTpho-encoder in extracting top-K sentences discussed in Section \ref{extractive_summarization}. Because our Bi-Encoder-Decoder architecture relies on the performance of the Bi-Encoder ability to extract most meaningful sentences with cosine-similarity from input documents, the performance of abstractive summarization in the decoder is strongly correlating with the performance of extractive summarization.
The results of two models ViT5\textsubscript{256-length} and ViT5\textsubscript{1024-length} are predictably different. The ViT5\textsubscript{256-length} model, which performs competitively in extractive summarization, has sequence length too small for the abstractive summarization generation tasks and achieves minor performance. Utilizing Bi-Encoder-Decoder architecture, ViT5\textsubscript{1024-length} outperforms other models on the extractive summarization which leads to its state-of-the-art performance on the abstractive summary generation. Outperforming other existing language models on both extractive summarization and abstractive summarization tasks, both ViT5\textsubscript{1024-length}'s encoder and decoder are effectively in learning monolingual Vietnamese representation in multi-document summarization. ViT5\textsubscript{1024-length} performances show that our proposed Bi-Encoder-Decoder architecture is effective in creating an end-to-end architecture to generate both extractive and abstractive summarization.
\input{ACLStudent2021/table/abstractive_result}


==> table/abstractive_result.tex <==
\begin{table}[hbt!]
\centering
\caption{Test result on VietnameseMDS Multi-Document Abstractive Summarization}

\begin{tabular}{l|ccc}
\hline
Models     & Rouge-1        & Rouge-2        & Rouge-L        \\ \hline
BARTpho    & 64.47          & 33.06          & 35.41          \\ \hline
mBART      &   {\ul 65.55}            &   35.97             &  38.36              \\ \hline
mT5        &     65.44           &   {\ul 40.26}             &  {\ul 40.56}        \\ \hline
% ViT5(256)  &                &                &                \\ \hline
ViT5\textsubscript{256-length} & 62.40 & 34.12 & 37.41 \\ \hline

ViT5\textsubscript{1024-length} & \textbf{69.36} \textbf{41.15} & \textbf{41.88} \\ \hline
\end{tabular}


\begin{tablenotes}
      \small
      \item \textit{Notes:} The best scores are in bold and second best scores are underlined.
\end{tablenotes}
\label{abstractive_result}
\end{table}

==> table/extractive_result.tex <==
\begin{table*}[hbt!]
\centering
\caption{Test results on VietnameseMDS Multi-Document Extractive Summarization}

\begin{tabular}{c|l|c|c|c}
% \toprule
\hline
\multicolumn{1}{l|}{}                                                                                & Models        & Rouge-1                                & Rouge-2    & Rouge-L        \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}BERT-Encoder\\ with \\ Embedding \\ Clustering\end{tabular}} & mBERT         & 77.26                              & 50.52      &  -  \\ 
                                                                                                     & PhoBERT\textsubscript{base}  & 77.07                              & 50.95  &   -     \\ 
                                                                                                     & PhoBERT\textsubscript{large} & 77.42                              & 50.89   &  -     \\ 
                                                                                                     & viBERT4news   & {\ul 77.44}                        & {52.01}    & - \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Bi-Encoder\\  with \\ Cosine-Similarity Scores \\ Clustering\end{tabular}}     & mBART       & 71.49         & {46.08}      & 42.39    \\ 
                                                                                                     & BARTpho     & 74.65         & \textbf{55.48} & \textbf{45.61}    \\ 
                                                                                                     & mT5        & 77.13       & {\ul 53.00}        &   43.86 \\
                                                                                                     & ViT5\textsubscript{256-length}     &     {75.52}        & {51.18}& {\ul 44.31}   \\ 
                                                                                                     & ViT5\textsubscript{1024-length}   & \textbf{77.47} & {53.47} & \textbf{45.44} \\ \hline
\end{tabular}


\begin{tablenotes}
\centering
      \small
      \item \textit{Notes:} The best scores are in bold and second best scores are underlined.
\end{tablenotes}
\label{extractive_result}
\end{table*}

==> table/model_stats.tex <==
\begin{table*}[hbt!]
\centering
\small
\begin{tabular}{@{}llll@{}}
\toprule
                          & ViT5\textsubscript{base 256-length} & ViT5\textsubscript{base 1024-length} & ViT5\textsubscript{large 1024-length} \\ \midrule
\# of parameters          & 220M                 & 220M                  & 738M       \\
\#of pre-train steps      & 1000000              & 1000000               & 1000000    \\
Batch size                & 128                  & 128                   & 256        \\
Pre-train sequence length & 256                  & 1024                  & 1024       \\
Finetune sequence length  & 1024                 & 1024                  & 1024       \\
Hardware                  & TPU v2-8             & TPU v2-8              & TPU v3-8   \\ \bottomrule
\end{tabular}
\caption{ViT5 Models Settings}

\label{model_stats}
\end{table*}








==> table/phoner_stats.tex <==
\begin{table*}[hbt!]
\centering
\caption{Statistics of PhoNER\_COVID19 Dataset}

\begin{tabular}{llccc}
\toprule
Entity              & Train & Valid & Test  & All   \\ \midrule
PATIENT\_ID         & 3240  & 1276  & 2005  & 6521  \\
NAME                & 349   & 188   & 318   & 855   \\
AGE                 & 682   & 361   & 582   & 1281  \\
GENDER              & 542   & 277   & 462   & 1281  \\
OCCUPATION          & 205   & 132   & 173   & 510   \\
LOCATION            & 5398  & 2737  & 4441  & 12576 \\
ORGANIZATION        & 1137  & 551   & 771   & 2459  \\
SYMPTION \& DISEASE & 1439  & 766   & 1136  & 3341  \\
TRANSPORTATION      & 226   & 87    & 193   & 506   \\
DATE                & 2549  & 1103  & 1654  & 5306  \\
\# entites          & 15767 & 7478  & 11735 & 34984 \\
\# sentences        & 5027  & 2000  & 3000  & 10027 \\ \midrule
\# avg of words     & \multicolumn{4}{c}{77}        \\ \bottomrule
\end{tabular}
\label{phoner_stat}
\end{table*}

==> table/results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\caption{Test result on Wikilingua}

\begin{tabular}{l|llll}
\hline
\multirow{2}{*}{Models}                                         & \multicolumn{4}{c|}{Vietnews}                                \\ \cline{2-5} 
                                                                & Rouge-1        & Rouge-2        & Rouge-L        & BERTScore \\ \hline
\begin{tabular}[c]{@{}l@{}}Transformer\\ (RND2RND)\end{tabular} & 57.56          & 24.25          & 35.53          &           \\ \hline
PhoBERT2RND                                                     & 57.6           & 24.18          & 35.5           &           \\ \hline
ViBERT2ViBERT                                                   & 59.75          & 27.29          & 36.79          &           \\ \hline
PhoBERT2PhoBERT                                                 & 60.37          & 29.12          & 39.44          &           \\ \hline
mBERT                                                           & 59.67          & 27.36          & 36.73          &           \\ \hline
mBART                                                           & 59.81          & 28.28          & 38.71          &           \\ \hline
mT5                                                             & 58.05          & 26.76          & 37.38          &           \\ \hline
BARTpho                                                         &                &                & 39.85          &           \\ \hline
ViT5 (256-length)                                               & \textit{61.85} & \textit{31.70} & \textit{41.70} &           \\ \hline
ViT5 (1024-length)                                              & \textbf{62.77} & \textbf{33.16} & \textbf{42.75} &           \\ \cline{1-4}
\end{tabular}

\begin{tablenotes}
      \small
      \item \textit{Notes:} The best scores are in bold and second best scores are underlined.
\end{tablenotes}
\label{result}
\end{table*}

==> table/vietnews.tex <==
\begin{table*}[hbt]
\centering
\caption{Test result on Vietnews}

\begin{threeparttable}
\begin{tabular}{l|lll}
\hline
\multirow{2}{*}{Models}                                         & \multicolumn{3}{c}{Vietnews}                                \\ \cline{2-4} 
                                                                & Rouge-1        & Rouge-2        & Rouge-L         \\ \hline
\begin{tabular}[c]{@{}l@{}}Transformer\\ (RND2RND)\end{tabular} & 57.56          & 24.25          & 35.53                   \\ \hline
PhoBERT2RND                                                     & 57.6           & 24.18          & 35.5                      \\ \hline
ViBERT2ViBERT                                                   & 59.75          & 27.29          & 36.79                     \\ \hline
PhoBERT2PhoBERT                                                 & 60.37          & 29.12          & 39.44                     \\ \hline
mBERT                                                           & 59.67          & 27.36          & 36.73                     \\ \hline
mBART                                                           & 59.81          & 28.28          & 38.71                     \\ \hline
mT5                                                             & 58.05          & 26.76          & 37.38                     \\ \hline
BARTpho                                                         &  61.14              & 30.31               & 40.15                    \\ \hline
ViT5\textsubscript{256-length}                                            & {61.85} & { 31.70} & {41.70}            \\ \hline
ViT5\textsubscript{1024-length}                                              & {\ul 62.77} & {\ul 33.16} & {\ul 42.75}            \\ \hline
ViT5\textsubscript{large}\textsubscript{1024-length}                                              & \textbf{63.16} & \textbf{34.05} & \textbf{43.46}   \\ \hline

\end{tabular}

\begin{tablenotes}
      \small
      \item \textit{Notes:} The best scores are in bold and second best scores are underlined.
\end{tablenotes}
\end{threeparttable}
\label{vietnews}

\end{table*}

==> table/vimds_stats.tex <==
\begin{table}[hbt!]
\centering
\caption{Statistics of VietnameseMDS Dataset}

\begin{tabular}{l|c}
\hline
Dataset      & VietnameseMDS \\ \hline
Clusters     & 200           \\
Documents    & 600           \\
References   & 400           \\
\# sentences & 9802          \\ \hline
\end{tabular}
\label{vimds_stats}
\end{table}

==> table/wikilingua_examples.tex <==
\begin{table*}[hbt!]
\centering
\caption{Example of results between ViT5 and BARTpho on Wikilingua Summarization Corpus}
\small
\begin{threeparttable}
\begin{tabular}{l|l|l|l}
\hline
\textbf{Content}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \multicolumn{1}{c|}{\textbf{Reference}}                                                                                                                                                                               & \multicolumn{1}{c|}{\textbf{ViT5}}                                                                                                                                                            & \multicolumn{1}{c}{\textbf{BARTpho}}                                                                                  \\ \hline
\small
\textbf{Vietnamese}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 &                                                                                                                                                                                                                       &                                                                                                                                                                                               &                                                                                                                       \\ \cline{1-1}
\begin{tabular}[c]{@{}l@{}}Nếu bạn thật sự đang cố gắng để cải\\ thiện điểm số của mình nhưng mọi \\chuyện vẫn không tiến triển, bạn nên\\ trò chuyện với thầy cô...\\ Nhiều thầy cô không thích cộng điểm\\ thêm, nhưng họ sẽ thông cảm cho bạn\\ nếu họ nhận thấy bạn đang cố gắng\\ hết mình để trở nên tốt hơn.\\ Nếu bạn thật sự gặp khó khăn, bạn \\ nên nhờ thầy cô hoặc trung tâm gia sư\\ của trường tìm kiếm gia sư...\\ Khi bạn học cùng người khác, bạn sẽ\\ tận dụng được mọi sự thông minh và\\ sự hiểu biết của bản thân để trở nên \\xuất sắc hơn...\\ Nếu bạn học bài trong môi trường\\ thực tế... bạn sẽ ghi nhớ thông tin một\\ cách tốt hơn... \\ Có khá nhiều công cụ trực tuyến giúp\\ giải thích tài liệu mà bạn đang cố\\ học...\end{tabular} & \begin{tabular}[c]{@{}l@{}}Tham khảo lời \\ khuyên của thầy cô. \\ Xin được cộng\\ điểm. \\ Thuê gia sư. \\ Học nhóm. \\ Cung cấp cho bản\\ thân bối cảnh cụ\\ thể. \\ Tìm kiếm công cụ\\ trực tuyến.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Trò chuyện với\\ giáo viên của bạn. \\ Xin cộng điểm \\ nếu cần. \\ Tìm gia sư. \\ Học cùng người \\ khác. \\ Tìm kiếm sự trợ\\ giúp trực tuyến.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gặp giáo viên. \\ Xin phép cộng\\ điểm. \\ Xin phép nộp \\ bài tập về nhà.\end{tabular}    \\ \hline
\small
\textbf{English Translation}&                                                                                                                                                                                                                       &                                                                                                                                                                                               &                                                                                                                       \\ \cline{1-1}

\small
\begin{tabular}[c]{@{}l@{}}If you're really trying to improve your\\ grades but things aren't  working, you\\ should talk to your teacher...\\ Many teachers don't like to add extra\\ points, but they will sympathize with \\you if they see that you are trying \\your best to be better...\\ If you really have difficulty, you \\should ask your teacher or the \\school' tutoring center to find a tutor.\\ When you study with others, you will\\ use all your intelligence and\\ understanding to become better...\\ If you study in a real environment... \\ you will remember the information \\ better... \\ There are quite a few online tools to\\ help explain the material you are\\ trying to learn...\end{tabular}                       & \small \begin{tabular}[c]{@{}l@{}}Ask for teachers' \\ advice.\\ Ask for grade\\changes.\\ Hire a tutor.\\ Study in groups.\\ Give yourself study\\ environment.\\ Search online tools.\end{tabular}                      & \small \begin{tabular}[c]{@{}l@{}}Chat with your \\ teachers.\\ Ask for grade\\ changes if needed.\\ Find a tutor.\\ Learn with others.\\ Seek help online.\end{tabular}                             & \small \begin{tabular}[c]{@{}l@{}}Meet the teacher.\\ Ask for grade \\ changes.\\ Ask to submit\\ the homework.\end{tabular} \\ \hline
\end{tabular}
\begin{tablenotes}
      \small
      \item The English Translation is manually created for general readers. The document is on the topic of improving score for students. ViT5 model creates a summary more accurate and has a close meaning to the reference summary.
\end{tablenotes}
\end{threeparttable}
\label{wikilingua_examples}
\end{table*}
